Frugal Byzantine Computing

Traditional techniques for handling Byzantine failures are expensive: digital signatures are too costly, while using $3f{+}1$ replicas is uneconomical ($f$ denotes the maximum number of Byzantine processes). We seek algorithms that reduce the number of replicas to $2f{+}1$ and minimize the number of signatures. While the first goal can be achieved in the message-and-memory model, accomplishing the second goal simultaneously is challenging. We first address this challenge for the problem of broadcasting messages reliably. We consider two variants of this problem, Consistent Broadcast and Reliable Broadcast, typically considered very close. Perhaps surprisingly, we establish a separation between them in terms of signatures required. In particular, we show that Consistent Broadcast requires at least 1 signature in some execution, while Reliable Broadcast requires $O(n)$ signatures in some execution. We present matching upper bounds for both primitives within constant factors. We then turn to the problem of consensus and argue that this separation matters for solving consensus with Byzantine failures: we present a practical consensus algorithm that uses Consistent Broadcast as its main communication primitive. This algorithm works for $n=2f{+}1$ and avoids signatures in the common-case -- properties that have not been simultaneously achieved previously. Overall, our work approaches Byzantine computing in a frugal manner and motivates the use of Consistent Broadcast -- rather than Reliable Broadcast -- as a key primitive for reaching agreement.

==> MI_NEB.tex <==

\renewcommand{\figurename}{Algorithm}
\begin{figure}[ht!]
    \caption{Fast Non-Equivocating Broadcast}
    \begin{lstlisting}[columns=fullflexible,breaklines=true, keywords={}]
Shared:
slots - @$n \times M \times n$@ array of "slots"; each slot is a 2-tuple (msg, sgn) of SWMR atomic registers, initialized to @$(\bot,\bot)$@.  

Sender code:
broadcast(k,m) {
    for all replicators and receivers r {
        send((k,m)) to r;}
    In the background {
        @$\sigma$@ = compute signature for m
        for all replicators and receivers r {
            send((k,@$\sigma$@)) to r;}
}   }

Replicator code:
two cursors: cur_copy, cur_copy_sign, initially 1
while (true) {
    for q in @$\Pi$@ {
        if received message m from q{ 
            slots[me,cur_copy,q].msg.write(m)
            cur_copy += 1   }
        if received signature sign from q {
            val = slots[me,cur_copy_sign,q].msg.read()
            if (val @$\neq$@ @$\bot$@ && sign @$\neq$@ @$\bot$@ && sign is a valid signature for val) {
                slots[me,cur_copy_sign,q].sgn.write(sign)
                cur_copy_sign += 1
            }     }   }   } @\Naama{Need to stop copying signatures if we receive a bad signature from the sender}@

Receiver code:
try_deliver(k,q) {
    upon receiving message m from q @\label{line:copy-m}@{
        msg = m }
    upon receiving signature @$\sigma$@ from q {
        sign = @$\sigma$@}
        
    if msg == @$\bot$@ {return @$\bot$@}
    others = scan(k,q) @\label{line:scan}@
    if (others[t].msg == msg for all t in @$\Pi$@) {
        return msg @\label{line:fast-return}@
    } else if (sign @$\neq$@ @$\bot$@) && (@$\nexists$@ t s.t. others[t].sgn is a valid signature for others[t].msg && others[t].msg @$\neq$@ msg) && (others contains f+1 signed copies of msg)) { @\label{line:slow-check}@
        return msg @\label{line:slow-return}@
    } else {
        return @$\bot$@    }
}

scan(k,q) {@\label{line:scan-start}@
    others = slots[t,k,q].(msg,sgn).read() for t in @$\Pi$@ @\label{line:fillOthers}@
    do {
        done = true @\label{line:doneT}@
        for (t in @$\Pi$@) {
            if (others[t] == @$\bot$@) {
                others[t] = slots[t,k,q].(msg,sgn).read(); @\label{line:updateOthers}@
                if (others[t] @$\neq$@ @$\bot$@) {
                    done = false @\label{line:doneF}@
                }     }       }
    } while (!done)
    return others
} @\label{line:scan-end}@
\end{lstlisting}
    \label{alg:fast-non-eq}
\end{figure}
\renewcommand{\figurename}{Figure}


==> MI_RB.tex <==
\begin{definition}[Reliable Broadcast]
	In \emph{reliable broadcast}, there is a designated process $p$ called the \emph{sender} that can broadcast any number of messages, such that the following conditions hold:
	\begin{enumerate}
		\item If $p$ is correct, then every correct process eventually delivers every message that $p$ broadcasts.
		\item If some correct process $q$ delivers message $m$ from $p$, then eventually every correct process delivers $m$ from $p$.
		\item If some correct process delivers a message $m$ from $p$, then $p$ broadcast $m$ at some earlier point in time.
	\end{enumerate}
\end{definition}


\renewcommand{\figurename}{Algorithm}
\begin{figure}[h]
	\caption{Fast Reliable Broadcast}
	\begin{lstlisting}[columns=fullflexible,breaklines=true]
SWMR Value[n,M,n]; //Initially, Value[j,k,i]=@$\bot$@. 
SWMR L1Proof[n,M,n]; //Initially, L1Proof[j,k,i]=@$\bot$@. 
SWMR L2Proof[n,M,n]; //Initially, L2Proof[j,k,i]=@$\bot$@. 
	
sender code:
    void broadcast (k,m){
        send (k,m) to all   }

Code @\texttt{for}@ replicator p
    next_s; //next index to deliver from sender. Initially, next_s=1
    state; //@$\in$@{WaitForSender,WaitForL1Proof,WaitForL2Proof}. Initially, state=WaitForSender
	
		
		upon receiving message msg from sender
		Write(Value[p,k,q], msg);
		
		In the background, compute
		@$\sigma$@ = sign(msg);
		Write(Value[p,k,q], @$\sigma$@)
		
		state = WaitForL1Proof;
	
		if (state == WaitForL1Proof) {
			checkedVals = @$\emptyset$@;
			for i @$\in \Pi$@{
				v = Read(Value[i,k,q]);@\label{line:readValCopies}@
				if (validateValue(v,my_val,k,i)) {checkedVals.add((i,v));} }
	
			if (size(checkedVals) @$>$@ n/2) {@\label{line:checkL1proof}@
				l1prf = sign(checkedVals);
				Write(L1Proof[p,k,q], l1prf);@\label{line:writel1prf}@
				read all L1 proofs;
				If there is no L1 proof that contradicts mine { Write(L1Proof[p,k,q].valid, true)
				} @\Naama{This part is way less formal than the rest. I think it might be better. Fix the rest, or fix this.}@
				state = WaitForL2Proof; }   }
	
		if (state == WaitForL2Proof){
			checkedL1Prfs = @$\emptyset$@;
				for i in @$\Pi$@{
					prf = Read(L1Proof[i,k,q]);@\label{line:readL1prf}@
					if (validateL1Prf(prf,my_val,k,i)) {checkedL1Prfs.add((i,prf));}}
	
			if (size(checkedL1Prfs) @$>$@ n/2) {
				l2prf = sign(checkedL1Prfs);
				Write(L2Proof[p,k,q], l2prf); }   } }@\label{line:writeL2proof1}@
	\end{lstlisting}
	\label{alg:fast-rb}
\end{figure}

%code for receiver
%	void try_deliver(q) {
%		k = next_s;
%		val = checkL2Proof(s,k);
%		if (val != null) {
%			deliver(k, val, s);@\label{line:deliver}@
%			next_s += 1;
%			state = WaitForSender;
%			return;	}
%		my_val = Read(Value[p,k,q]);


\begin{figure}[h]
	\caption{Helper functions for Fast Reliable Broadcast algorithm}
\begin{lstlisting}[firstnumber=52]
value checkL2proof(q,k) {
	for i@$\in \Pi$@ { 
		proof = Read(L2Proof[i,k,q]);@\label{line:readL2proof}@
		if (proof != @$\bot$@){
			val = first value in proof;	}
		if (proof != @$\bot$@ && validateL2Prf(proof,val,k,i)) {
			Write(L2Proof[p,k,q],proof); @\label{line:writeL2proof2}@
			return val; }   }
	return null;    }
	
bool validateValue(v, val, k, q){
	if (v == val && sValid(q,v) && key == k){
		return true; }
	return false;	}
	
bool validateL1Prf(proof, val, k, q){
    if (!proof.valid || size(proof) @$\leq$@ n/2) { return false; }
	for each (i,(v, s)) @$\in$@ proof {
		if (!validateValue(v,val,k,q) || !sValid(i, (v,s)){
			return false;	} 	}
	return true;	}

bool validateL2Prf(proof, val, k, q){
    if (size(proof) @$\leq$@ n/2) { return false; }
	for each (i,(l1prf,s)) @$\in$@ proof {
		if (!validateL1Proof(l1prf,val,k,s) || !sValid(i, (l1prf, s))){
			return false;}	} 	}
	return true;	}
\end{lstlisting}
\label{alg:rb-help}
\end{figure}

\Naama{Pseudocode of validation is a bit inaccurate. Need to carefully check which signatures are being validated when checking the proofs, match the ids properly.}

==> lowerbounds.tex <==
\section{Lower Bounds on Broadcast Algorithms}\label{sec:lowerbounds}

We show lower bounds on the number of signatures required to solve \neb{} and \rb{} while tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures in our model.

At a high level, our lower bound proofs rely on \emph{indistinguishability} arguments. That is, assuming an algorithm that breaks our bounds exists, we present executions in which correct receivers must deliver different values, and then argue that these executions are indistinguishable to the receivers. Thus, any such algorithm would inevitably break the properties of broadcast in some execution. 

Recall that we allow processes to communicate through both shared memory read/write registers and message passing. Furthermore, we present our bounds in terms of three different process roles; the \emph{sender} is the only process that can call \texttt{broadcast}, and, if it is correct, only sends one value. The \emph{receivers} are the only processes that call \texttt{deliver}, and are meant to model short-lived clients in a replicated system. 
%\Naama{Is it ok to assume receivers don't send messages and write? I think we don't strictly need that assumption, but it makes the proofs cleaner.}
%MKA: ok
Finally, the \emph{replicators} represent all processes in the system. We allow up to $f$ of the $n$ replicators to be Byzantine; unless stated otherwise, our bounds are in terms of the number of replicator signatures. This model is more general that the standard model, and is equivalent to the standard model if all processes play all three roles. Thus, our results apply for the standard model as well.

%To argue about such scenarios in our model, which allows communication both through message passing and shared memory, we make use of the following notion of a Byzantine process \emph{portraying} an execution to some subset of the processes.

%\begin{definition}
%Consider an execution $E$ and a process $p$. Let $e_i$ be $p$'s $i$th step in $E$.
%We say that a process $p$ \emph{portrays} execution $E$ to a set of processes $S$ starting at time $t$ if, for each $i$, 
%\begin{itemize}
%    \item If $e_i$ was accessing shared memory that some process in $S$ can access, or sending a message to some process in $S$, then $p$'s $i$th step after time $t$ is $e_i$.
%    \item Otherwise, $p$'s $i$th step after time $t$ is a no-op.
%\end{itemize}
%\end{definition}

%That is, if $p$ portrays an execution $E$ to a set $S$ of processes, then in everything visible to $S$, $p$ acts as if it is experiencing execution $E$. However, $p$ does not communicate with processes in $\Pi \setminus S$ in communication channels that are not accessible to $S$. In particular, it doesn't send any messages to any process in $\Pi \setminus S$.

We first show that \neb{} requires at least a sender signature. To do so, the idea is to consider two non-overlapping sets $S_1$ and $S_2$, of size $f$ each, and let the remaining process be $p$. Intuitively, we construct different executions in which $p$ always acts as if it received $v$ from the sender, and processes in $S_1$ always behave as if they received $v'$ from the sender. 
\Naama{Continue intuition.}

\begin{lemma}\label{lem:onesig}
Any solution for the \neb{} problem on RDMA tolerating up to $f = \lfloor (n-1)/2 \rfloor$ replicator failures must use at least one signature in some execution.
\end{lemma}

\begin{proof}
Assume by contradiction that there exists an algorithm $A$ that solves \neb{} on RDMA in a system with $n\geq 2f+1$ replicators, and does not use any signatures. 
Consider a system with $n = 2f+1$ processes, and partition the replicators in the system into 3 subsets: $S_1$, $S_2$, and $p_1$, where $S_1$ contains the sender, $\vert S_1 \vert = f$, $\vert S_2 \vert = f$, and $p_1$ contains a single process.
Consider the following scenarios.

\textsc{Scenario 1.} Processes in $S_1$ and $p_1$ are correct, and processes in $S_2$ are faulty, and do not participate. The sender is correct and sends value $v$ to all processes. Then, since the sender is correct and $A$ is a correct algorithm, eventually processes in $S_1$ and $p_1$ must deliver $v$. 
%Let $State(p_1)$ be the state of all registers in the set 
%$$R_{p_1} = \{r\in R \vert p_1 \text{ was the last process that wrote on } r \text{ before } t\}$$.

%$$R_{p_1} = \{r\in R \vert p_1 \text{ was the last process that wrote on } r \text{ before processes in } S_1 \text{ and } p_1 \text{terminated}\}$$.

\textsc{Scenario 2.} $p_1$ is faulty, processes in $S_1$ and $S_2$ are correct. The sender is correct and sends value $v'$ to everyone. Initially, only $p_1$ takes steps, and it sends all messages and writes all values it did in Scenario 1.
%$p_1$ writes on all registers in $R_{p_1}$ such that they are in state $State(p_1)$ as defined in scenario 1. Furthermore, it sends all messages that it sent in scenario 1. 
Afterwards, processes in $S_1$ and $S_2$ start their execution. Then, by the correctness of $A$, all correct processes must deliver $v'$. 
%Assume $r_1$ does not participate, and let the first receiver that delivered $v'$ be $r_2 \neq r_1$.
%processes in $S_1$ and $S_2$ must eventually deliver $v'$.


\textsc{Scenario 3.} Processes in $S_1$ are faulty, %\dalia{given $|S_1|\geq f$, can this be that all processes in $S_1$ are faulty?}, 
the rest are correct. The sender is faulty and sends value $v$ to everyone in $p_1$ and $S_1$, and value $v'$ to everyone in $S_2$. 
%Furthermore, assume all messages from $r_1$ are arbitrarily delayed. 
$S_2$ are delayed and $S_1$ act as follows: in all messages sent to $p_1$, and everything written on shared memory, they act identically to their behavior in scenario 1. However, they do not send any messages to $S_2$ at this point. Note that this scenario is indistinguishable
to $p_1$ from scenario 1, so it eventually sends all messages and writes all values it did in scenario 1, and delivers $v$. 
Once this happens, processes in $S_1$ erase all values in all registers in which the last write so far was done by a process in $S_1$. 
%such that $p_1$ did not write in them in Scenario 2. 
Now, processes in $S_2$ wake up, and processes in $S_1$ act as they did in scenario 2. $p_1$ pauses for arbitrarily long.
%, but do not send messages to $p_1$. Furthermore, all messages from $p_1$ to processes in $S_2$ after $p_1$ delivers are arbitrarily delayed.

Note that this scenario is indistinguishable from scenario 2 to processes in $S_2$. Therefore, processes in $S_2$ eventually deliver $v'$. However, since $p_1$ delivered $v$,
%since $p_1$ was correct and delivered $v$ 
this violates the consistency property of \neb.
\end{proof}

\rmv{
\begin{proof}
Assume by contradiction that there exists an algorithm $A$ that solves \neb{} on RDMA in a system with $n\geq 2f+1$ replicators, and does not use any signatures. 
Consider a system with $n = 2f+1$ replicators, and partition the replicators in the system into 3 subsets: $S_1$, $S_2$, and $p_1$, where $\vert S_1 \vert = f$, $\vert S_2 \vert = f$, and $p_1$ contains a single process.
Consider the following scenarios.

\textsc{Scenario 1.} Processes in $S_1$ and $p_1$ are correct, and processes in $S_2$ are faulty, and do not participate. The sender is correct and sends value $v$ to all processes. Then, since the sender is correct and $A$ is a correct algorithm, eventually some correct receiver must deliver $v$. Let the time at which a receiver delivers $v$ be $t$, and let the receiver that delivered be $r_1$. %processes in $S_1$ and $p_1$ must terminate. 
%Let $State(p_1)$ be the state of all registers in the set 
%$$R_{p_1} = \{r\in R \vert p_1 \text{ was the last process that wrote on } r \text{ before } t\}$$.

%$$R_{p_1} = \{r\in R \vert p_1 \text{ was the last process that wrote on } r \text{ before processes in } S_1 \text{ and } p_1 \text{terminated}\}$$.

\textsc{Scenario 2.} $p_1$ is faulty, processes in $S_1$ and $S_2$ are correct. The sender is correct and sends value $v'$ to everyone. Initially, only $p_1$ takes steps, and it sends all messages and writes all values it did in Scenario 1.
%$p_1$ writes on all registers in $R_{p_1}$ such that they are in state $State(p_1)$ as defined in scenario 1. Furthermore, it sends all messages that it sent in scenario 1. 
Afterwards, processes in $S_1$ and $S_2$ start their execution. Then, by the correctness of $A$, all correct receivers must deliver $v'$.  Assume $r_1$ does not participate, and let the first receiver that delivered $v'$ be $r_2 \neq r_1$.
%processes in $S_1$ and $S_2$ must eventually deliver $v'$.


\textsc{Scenario 3.} Processes in $S_1$ are faulty, %\dalia{given $|S_1|\geq f$, can this be that all processes in $S_1$ are faulty?}, 
the rest are correct. The sender is faulty and sends value $v$ to everyone in $p_1$ and $S_1$, and value $v'$ to everyone in $S_2$. 
%Furthermore, assume all messages from $r_1$ are arbitrarily delayed. 
$S_2$ are delayed and $S_1$ act as follows: in all messages sent to $p_1$ and $r_1$, and everything written on shared memory, they act identically to their behavior in scenario 1. However, they do not send any messages to $S_2$ at this point. Note that this scenario is indistinguishable
to $p_1$ from scenario 1, so it eventually sends all messages and writes all values it did in scenario 1. %puts the registers in $R_{p_1}$ in state $State(p_1)$.
This is now indistinguishable from scenario 1 at time $t$ to receiver $r_1$, so it eventually delivers $v$. %some receiver eventually delivers $v$. 
Once this happens, processes in $S_1$ erase all values in all registers such that $p_1$ did not write in them in Scenario 2. Now, processes in $S_2$ wake up, and processes in $S_1$ act as they did in scenario 2, but do not send messages to $p_1$. Furthermore, all messages from $p_1$ to processes in $S_2$ after $r_1$ delivers are arbitrarily delayed.

Note that this scenario is indistinguishable from scenario 2 to receiver $r_2$. Therefore, $r_2$ eventually delivers $v'$. However, since another receiver $r_1$ delivered $v$,
%since $p_1$ was correct and delivered $v$ 
this violates the consistency property of \neb.
\end{proof}
}

Since any solution to \rb solves \neb, Lemma~\ref{lem:onesig} also applies to \rb.

We now show a separation between \neb{} and \rb{}. In particular, note that Algorithm~\ref{alg:fast-non-eq} solves \neb{} with just one signature, from the sender. We show that such a solution is impossible for the \rb{} problem. In fact, we show a  stronger result: any solution of the \rb{} problem must have some execution in which at least $2f$ processes create signatures.

%Intuitively, the proof of this result is very similar to the proof of the previous result. However, because the sender may now sign messages, we cannot argue indistinguishability between two scenarios such that in one of them the sender is correct, in the other it is faulty, and some process sees both values reported by others. This makes the proof a bit more complicated. Luckily, we can rely on the increased requirements of solving \rb{} as opposed to \neb; now, in every execution in which some correct process delivers, all correct processes must deliver, even if they recognize that the sender is faulty.

We categorize algorithms $A$ solving \rb{} into two groups, depending on whether there is some execution of $A$ in which all $n$ replicators sign messages. Clearly, algorithms that do have such executions trivially satisfy the bound we are trying to obtain, so we focus only on the algorithms that do not have such executions.

The proof is constructed in three stages. 
Firstly, we show that, for every algorithm $A$ that has no execution in which all processes sign, \emph{all} executions of $A$ must have at most $n-f-1$ correct processes that produce signatures. This is easy to prove, by considering that it is always possible to extend any execution such that $f$ additional (Byzantine) processes sign. Thus, if the number of correct signers plus the number of Byzantine processes adds up to $n$, we can produce an execution in which all processes sign.


\begin{lemma}\label{lem:manydontsign}
Let $A$ be an algorithm solving \rb{} on RDMA tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures,
such that no execution of $A$ has all $n$ processes signing.
%\mka{all $n$ -> all correct?}
Then in all executions of $A$, there must be at most $n-f-1$ correct processes that sign.
\end{lemma}

\begin{proof}
Assume by contradiction that this there is an algorithm $A$ solving \rb{} on RDMA tolerating $f = \lfloor (n-1)/2 \rfloor$ failures, such that no execution of $A$ has all $n$ processes signing, but there is some execution $E$ of $A$ in which at least $n-f$ correct processes sign. Let $S$ be the set of correct processes that sign in $E$; by assumption $|S|\geq n-f$.

Now consider the following extension $E'$ of $E$, in which all processes in $\Pi\setminus S$ are Byzantine (this is possible, since $|\Pi\setminus S| \leq f$). All processes execute $E$, with the Byzantine processes behaving correctly, until all processes in $S$ sign some value. Then have all processes in $\Pi\setminus S$ sign some value as well. In this execution, all $n$ processes signed, contradicting our assumption on $A$.
%
% Then let the processes in $\Pi\setminus B$ be Byzantine, and the rest be correct. Consider the following execution: All processes execute $E$, with the Byzantine processes behaving correctly, until all processes not in $B$ sign some value. 
\end{proof}

In the next stage of the proof, we show that there must be many executions in which at least one process produces a signature. More specifically, we show that in an execution $E$ in which (1)  not all processes participate, (2) the sender is correct, and (3) Byzantine processes only fail by crashing, there must be at least one signature in addition to a possible initial signature from the sender. The proof of this lemma uses an indistinguishability argument, and relies on the fact that there can't be too many signatures, given Lemma~\ref{lem:manydontsign}.

\begin{lemma}\label{lem:atleastonesig}
Let $A$ be an algorithm solving \rb{} on RDMA tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures, such that no execution of $A$ has all $n$ processes signing.
Then in all executions of $A$ in which at least $n-2f$ processes crash initially, 
%most $n-1$ processes participate, 
Byzantine processes only fail by crashing, and the sender is correct, at least one process signs, in addition to a possible initial sender signature.
%at least one replicator signs.
\end{lemma}

%\igor{In the lemma statement and proof, the word "participate" might be slightly confusing. Saying that n-1 processes participate might make it sound as if there are n-1 processes in the system, which is not what is meant (I think). Would it make sense to say that "at least 1 processes crashes initially" instead of "at most n-1 processes participate"?}

\begin{proof}
Assume by contradiction that there exists an algorithm $A$ such that $A$ satisfies all of the conditions outlined in the lemma, but there is some execution in $A$ in which the sender is correct and possibly signs its first message, Byzantine processes only fail by crashing, %\igor{and only n-1 processes participate} 
and at least $n-2f$ processes crash initially,
but no correct process produces a signature after the initial message of the sender.
%\igor{I am sure that we use the fact that no replicator signs in $E$ somewhere in the proof, but this is never made explicit. I feel like using this assumption explicitly would help with the clarity of the proof.}
Let $E$ be that execution, $C$ be the set of processes that participate in $E$, and $\Pi \setminus C$ be the set of faulty processes that crash from the start. Without loss of generality, let $v$ be the value that the sender sends to all processes in execution $E$.
%
Consider the following Scenarios:

\textsc{Scenario 1.} $E$ is the execution that occurs. Since the sender is correct, eventually all correct processes deliver $v$. We pause $E$ at the time at which the first process delivers. 
%\textsc{Scenario 1.} $E$ is the execution that occurs. Since the sender is correct, eventually some receiver delivers $v$. We pause $E$ at the time at which the first receiver delivers. Let $r_1$ be this receiver.

\textsc{Scenario 2.} The same set of processes, $C$, participate. All processes in $C$ are correct. The sender is still correct, but this time, it sends $v'$ to all.
Let $S \subset C$ be a set of processes such that (1) $|S| = f$, and (2) the set of processes that sign any message in this execution is a subset of  $S$. Note that by
Lemma~\ref{lem:manydontsign}, since $A$ has no execution in which $n$ processes sign, the number of processes that sign messages is $\leq f$, therefore the set $S$ exists. 
Eventually, all correct processes must deliver $v'$, since the sender is correct. 
%The scenario ends when the first receiver $r_2$ such that $r_2 \neq r_1$ delivers.
%Eventually, some receiver must deliver $v'$, since the sender is correct. The scenario ends when the first receiver $r_2$ such that $r_2 \neq r_1$ delivers.

%\igor{(1) If we take the most general case in which $n$ can be strictly larger than $2f+1$, the proof doesn't work anymore; this is because we need both $S$ and $T$ to be Byzantine in some scenario, and thus their sizes need to be at most $f$. But if $|S|+|T|=n-1>2f$, that is impossible. But this is not a big problem: we can just make all the lemmas refer to the case where $n=2f+1$; I don't feel like this weakens them too much. Or perhaps we can replace $p$ with a set of $n-2f$ processes instead. (2) In addition to assuming that $n=2f+1$, we actually need an additional assumption: we need $|S|=|T|=f$, otherwise their sizes cannot add up to $n-1=2f$. But this last part can be easily fixed by replacing "Let the set of processes that sign any message in this execution be $S \subset C$" with "Let $S$ be a set of $f$ processes which includes all processes that sign any message in this execution ($S$ exists by Lemma 5.2)."}


\textsc{Scenario 3.} Processes in $S$ are Byzantine, and the rest are correct.
%processes in $T = C\setminus S$ and $p$ are correct. 
The sender is faulty, and sends $v$ to correct processes, and sends both values to Byzantine processes. Initially, the execution proceeds identically to $E$, except that processes in $S$ 
%do not send messages to receivers other than $r_1$, and 
do not send messages to any process in $\Pi \setminus C$.
Note that since in $E$, any Byzantine process only failed by crashing, the correct processes in $T = C \setminus S$ can get to the same state the were in in Scenario 1, even if some of them were Byzantine in $E$. 
This scenario is so far indistinguishable to 
processes in $T = C \setminus S$ from Scenario 1.
%, so they eventually deliver $v$. 
Note that at least one process $p_t \in T$ was correct in Scenario 1, since all processes in $\Pi \setminus C$ were faulty, and there must have been at least $f+1$ correct processes in Scenario 1. So, eventually, $p_t$ delivers $v$. We pause the execution at this point. Note that for all processes in $T$, the messages they sent and wrote on shared memory up to this point are identical to those in Scenario 1.
%$r_1$ from Scenario 1, so $r_1$ eventually delivers $v$.

After $p_t$ delivers $v$, we pause all processes in $T$, and processes in $S$ change their states to be identical to their state at the end of Scenario 2. They can do so since no one in $T$ produced signatures in Scenario 2. Furthermore, processes in $S$ send all messages they did in Scenario 2.
%, with the exception of those that they sent to any process in $T$. %, and those sent to $r_1$.
At this point, we let the rest of the processes (in $\Pi \setminus C$) wake up and do whatever the protocol dictates.
Eventually, these processes must deliver $v$, since $p_t$ delivered $v$.
%Then any receiver that observes this state must deliver $v$, since $r_1$ already delivered $v$.

\textsc{Scenario 4.} Processes in $T$ are Byzantine, and the rest are correct. 
%processes in $S$ and $p$ are correct. 
The sender is faulty and sends $v'$ to processes in $S$, $v$ to those in $\Pi \setminus C$, %$\setminus \{S\cup T \}$
and both values to the Byzantine processes. Initially, the execution proceeds exactly like the execution in Scenario 2,  except that processes in $T$ 
%do not send messages to receivers other than $r_2$, and 
do not send messages to any process in $\Pi \setminus C$.
%
This scenario is so far indistinguishable to processes in $S$ from Scenario 2, so they eventually deliver $v'$.
%$r_2$ from Scenario 2, so $r_2$ eventually delivers~$v'$.

At this point, processes in $S$ are paused, and processes in $T$ put themselves in the state they were in at the end of Scenario 1. They can do so because in Scenario 1, no process signed, and in particular, there were no signatures by any process in $S$. 
Furthermore, processes in $T$ send all messages they did in Scenario 1.
%, with the exception of those that they sent to any process in $S$, and those sent to $r_2$.
This state is indistinguishable to processes in $\Pi \setminus C$ from the state in Scenario 3 before processes in $\Pi \setminus C$ woke up. We now let those processes wake up, and they must take the same steps they did in Scenario 3, since they cannot distinguish between the two executions.
Furthermore, since this scenario is indistinguishable from Scenario 3 to $\Pi \setminus C$, they must eventually deliver $v$, contradicting agreement.
%any receiver observing this state must deliver $v$, contradicting agreement.
\end{proof}

\begin{lemma}\label{lem:atleastonesig-sendersigns}
Let $A$ be an algorithm solving \rb{} on RDMA tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures, such that no execution of $A$ has all $n$ processes signing.
Then in all executions of $A$ in which the sender $s$ is correct and signs initially, at least $2$ processes crash initially, 
%most $n-1$ processes participate, 
Byzantine processes only fail by crashing, at least one process signs, in addition to the initial sender signature.
%at least one replicator signs.
\end{lemma}

%\igor{In the lemma statement and proof, the word "participate" might be slightly confusing. Saying that n-1 processes participate might make it sound as if there are n-1 processes in the system, which is not what is meant (I think). Would it make sense to say that "at least 1 processes crashes initially" instead of "at most n-1 processes participate"?}

\begin{proof}
Assume by contradiction that there exists an algorithm $A$ such that $A$ satisfies all of the conditions outlined in the lemma, but there is some execution in $A$ in which the sender is correct and signs its first message, Byzantine processes only fail by crashing, 
and at least $2$ processes crash initially,
but no correct process produces a signature after the initial message of the sender.
%\igor{I am sure that we use the fact that no replicator signs in $E$ somewhere in the proof, but this is never made explicit. I feel like using this assumption explicitly would help with the clarity of the proof.}
Let $E$ be that execution, $C$ be the set of processes that participate in $E$ ($|C|=n-2$), and $\Pi \setminus C$ be the set of faulty processes that crash from the start. Without loss of generality, let $v$ be the value that the sender sends to all processes in execution $E$.
%
Consider the following Scenarios:

\textsc{Scenario 1.} $E$ is the execution that occurs. Since the sender is correct, eventually all correct processes deliver $v$. We pause $E$ at the time at which the first process delivers. 
%\textsc{Scenario 1.} $E$ is the execution that occurs. Since the sender is correct, eventually some receiver delivers $v$. We pause $E$ at the time at which the first receiver delivers. Let $r_1$ be this receiver.

\textsc{Scenario 2.} The same set of processes, $C$, participate. All processes in $C$ are correct. The sender is still correct, but this time, it sends $v'$ to all.
Let $S \subset C$ be a set of processes such that (1) $|S| = f$, and (2) the set of processes that sign any message in this execution is a subset of $S$. Note that by
Lemma~\ref{lem:manydontsign}, since $A$ has no execution in which $n$ processes sign, the number of processes that sign messages is $\leq f$, therefore the set $S$ exists. Since we assume that the sender $s$ signs its first message, $s$ must be in the set $S$.
Eventually, all correct processes must deliver $v'$, since the sender is correct. 
%The scenario ends when the first receiver $r_2$ such that $r_2 \neq r_1$ delivers.
%Eventually, some receiver must deliver $v'$, since the sender is correct. The scenario ends when the first receiver $r_2$ such that $r_2 \neq r_1$ delivers.

%\igor{(1) If we take the most general case in which $n$ can be strictly larger than $2f+1$, the proof doesn't work anymore; this is because we need both $S$ and $T$ to be Byzantine in some scenario, and thus their sizes need to be at most $f$. But if $|S|+|T|=n-1>2f$, that is impossible. But this is not a big problem: we can just make all the lemmas refer to the case where $n=2f+1$; I don't feel like this weakens them too much. Or perhaps we can replace $p$ with a set of $n-2f$ processes instead. (2) In addition to assuming that $n=2f+1$, we actually need an additional assumption: we need $|S|=|T|=f$, otherwise their sizes cannot add up to $n-1=2f$. But this last part can be easily fixed by replacing "Let the set of processes that sign any message in this execution be $S \subset C$" with "Let $S$ be a set of $f$ processes which includes all processes that sign any message in this execution ($S$ exists by Lemma 5.2)."}


\textsc{Scenario 3.} Processes in $S$ are Byzantine, and the rest are correct.
%processes in $T = C\setminus S$ and $p$ are correct. 
The sender sends $v$ to correct processes, and sends both values to Byzantine processes. Initially, the execution proceeds identically to $E$, except that processes in $S$ 
%do not send messages to receivers other than $r_1$, and 
do not send messages to any process in $\Pi \setminus C$.
Note that since in $E$, any Byzantine process only failed by crashing, the correct processes in $T = C \setminus S$ can get to the same state the were in in Scenario 1, even if some of them were Byzantine in $E$. 
This scenario is so far indistinguishable to 
processes in $T = C \setminus S$ from Scenario 1.
%, so they eventually deliver $v$. 
Note that at least one process $p_t \in T$ was correct in Scenario 1, since all processes in $\Pi \setminus C$ were faulty, and there must have been at least $f+1$ correct processes in Scenario 1. So, eventually, $p_t$ delivers $v$. We pause the execution at this point. Note that for all processes in $T$, the messages they sent and wrote on shared memory up to this point are identical to those in Scenario 1.
%$r_1$ from Scenario 1, so $r_1$ eventually delivers $v$.

After $p_t$ delivers $v$, we pause all processes in $T$, and processes in $S$ change their states to be identical to their state at the end of Scenario 2. They can do so since no one in $T$ produced signatures in Scenario 2. Furthermore, processes in $S$ send all messages they did in Scenario 2.
%, with the exception of those that they sent to any process in $T$. %, and those sent to $r_1$.
At this point, we let the rest of the processes (in $\Pi \setminus C$) wake up and do whatever the protocol dictates.
Eventually, these processes must deliver $v$, since $p_t$ delivered $v$.
%Then any receiver that observes this state must deliver $v$, since $r_1$ already delivered $v$.

\textsc{Scenario 4.} Processes in $\lbrace s \rbrace \cup T$ are Byzantine (this is possible since $|T| = |C \setminus S| = n - 2 - f = f-1$), and the rest are correct. 
%processes in $S$ and $p$ are correct. 
The sender $s$ sends $v'$ to processes in $S \setminus \lbrace s \rbrace$, $v$ to those in $\Pi \setminus C$, %$\setminus \{S\cup T \}$
and both values to the Byzantine processes. Initially, the execution proceeds exactly like the execution in Scenario 2,  except that processes in $\lbrace s \rbrace \cup T$ 
%do not send messages to receivers other than $r_2$, and 
do not send messages to any process in $\Pi \setminus C$.
%
This scenario is so far indistinguishable to processes in $S \setminus \lbrace s \rbrace$ from Scenario 2, so they eventually deliver $v'$.
%$r_2$ from Scenario 2, so $r_2$ eventually delivers~$v'$.

At this point, processes in $S$ are paused, and processes in $T$ put themselves in the state they were in at the end of Scenario 1. They can do so because in Scenario 1, no other process signed except the sender, and in particular, there were no signatures by any process in $S \setminus \lbrace s \rbrace$. 
Furthermore, processes in $T$ send all messages they did in Scenario 1.
%, with the exception of those that they sent to any process in $S$, and those sent to $r_2$.
This state is indistinguishable to processes in $\Pi \setminus C$ from the state in Scenario 3 before processes in $\Pi \setminus C$ woke up. We now let those processes wake up, and they must take the same steps they did in Scenario 3, since they cannot distinguish between the two executions.
Furthermore, since this scenario is indistinguishable from Scenario 3 to $\Pi \setminus C$, they must eventually deliver $v$, contradicting agreement.
%any receiver observing this state must deliver $v$, contradicting agreement.
\end{proof}

Finally, using the result of Lemma~\ref{lem:atleastonesig}, we construct an execution in which $f$ correct replicators produce signatures. This is done by repeatedly causing one correct replicator to be poised to sign some value, and then pausing it and letting the execution proceed until another process is poised to sign.

\begin{lemma}\label{lem:atleastfsigs}
Every algorithm that solves \rb{} on RDMA while tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures has some execution in which at least $f$ correct processes sign.
\end{lemma}

\begin{proof}
If $A$ has an execution in which all $n$ processes sign, then clearly, that execution includes the signatures of $f+1$ correct processes, satisfying our lemma. 

We therefore consider only algorithms that have no execution in which all $n$ processes sign. Let $A$ be such an algorithm, and consider the following execution of $A$.

All processes are correct, and so is the sender. The sender sends $v$ to all.

Initially, processes $p_1 \ldots p_{f+1}$ participate, and the rest are silent. By Lemma~\ref{lem:atleastonesig}, some process in $p_1 \ldots p_{f+1}$ must eventually sign. Without loss of generality, let $p_1$ be the first process that signs in this execution. We let the execution run until $p_1$'s next step is to make its signature visible. At this point, we pause $p_1$, and let $p_{f+2}$ begin executing. Again by Lemma~\ref{lem:atleastonesig}, eventually some process in $p_2 \ldots p_{f+2}$ will create a signature and make it visible. We let the first process to do so reach the state in which it is about to make its signature visible, and then pause it, and let $p_{f+3}$ start executing.

We continue in this way, each time getting to a state where $k$ processes have participated, and $k-f$ are poised to sign. Lemma~\ref{lem:atleastonesig} can be used until we get to $k= n-1$.

At that point, we have a state in which $f$ processes are poised to make their signatures visible. We now let these $f$ processes each take one step. Thus, we have constructed an execution of $A$ in which $f$ correct processes signed.
\end{proof}

The final theorem is an immediate corollary of Lemma~\ref{lem:atleastfsigs}, using the fact that we can extend the execution of Lemma~\ref{lem:atleastfsigs} with $f$ Byzantine signatures.

\begin{theorem}
Every algorithm that solves \rb{} on RDMA while tolerating up to $f = \lfloor (n-1)/2 \rfloor$ failures has some execution in which at least $2f$ processes sign.
\end{theorem}

\begin{proof}
This theorem is easily implied by Lemma~\ref{lem:atleastfsigs}. For every algorithm $A$ that solves \rb{} on RDMA while tolerating $f < n/2$ failures, either $A$ has an execution in which $n$ processes sign, or, by Lemma~\ref{lem:atleastfsigs}, it has an execution in which at least $f$ correct processes sign. Consider the latter case, and let $E$ be such an execution of $A$. Then let $E$ run until all $f$ correct processes sign, and now make the remaining $f$ Byzantine processes append their own signatures. We thus get an execution of $A$ in which $2f$ replicators signed, as desired.
\end{proof}


\rmv{
\dalia{attempt-zone(?)}
\textit{If following assumption is okay: it's fine for a byzantine sender to delay its message sent to one correct replicator initially (said otherwise, delay 1 correct replicator from hearing from a byzantine sender for a period of time); then:}
let s be the sender
we assume 1 correct process (that is not the sender) does not append its own signature
$|A|=|B| = f-2$
Sc.1:
s, A, b  = correct
B, a = faulty
Sender sends v signed to all 
Let a,B crash 
It then looks like:
s has v with its signature
A has v with sender's signature and their own signatures 
b has v with sender's signature only (but not its own - assumption, the replicator that does not sign)
a, B have 'crashed'
//let 1 deliver; 1 more corr be delayed finally get sender s msg (also no sign?; incr statement to 2?)

Sc.2: 
s, B, a = correct
A, b = faulty
s has v' with its own signature
B has v' with sender's signature and their own signature 
a has v' with sender's signature but not one of a (assumption; 1 replicator that does not sign) 
A, b have 'crashed'

Sc.3.
A, a = correct
s, B, b = faulty
s has v signed by itself 
A has v with signature of sender and own signatures 
let a be delayed, a is still waiting for a sender's message (+ the assumption that 1 correct proc that does not sign)
B has 'crashed' 
b has v signed by sender but not by itself
Scenario is equivalent to Sc.1, 1 delivers v
B suddenly not crashed anymore, set their value to v' signed by sender and themselves
now let a finally receive a sender's message, v' signed by sender
//alternative to this step is b switches to empty (did not sign this round so it's okay)
Any proc must del v

Sc.4.
B, b = correct
s, A, a = faulty
s has v' signed by itself 
B has v' signed by itself and their signature
let b be delayed, b is still waiting for sender's message (+ aspt 1 corr does not sign)
A - 'crashed'
a has v' signed by sender yet not itself
Same as Sc.2; 1 delivers v'
Now A are suddenly not crashed, set to v signed by sender and their own signs
let b finally receive sender's message, v signed by the sender 
//alternative a switches to empty (never appended its own signature this round so fine)
Now same as scenario 3

//new attempt
$|A|=|B| = f-2$
let 2 correct not sign 
Sc.1:
s, A, b, q2  = correct
B, a, q1 = faulty
Sender sends v signed to all 
Let a,B,q1 crash 
It then looks like:
s has v with its signature
A has v with sender's signature and their own signatures 
b has v with sender's signature only (but not its own - assumption, the replicator that does not sign)
a, B,q1 have 'crashed'
//let 1 deliver; 1 more corr be delayed finally get sender s msg (also no sign?; incr statement to 2?)
q2 delayed - finally gets v w sender's signature (but not its own, assumption)

Sc.2: 
s, B, a, q1 = correct
A, b, q2 = faulty
s has v' with its own signature
B has v' with sender's signature and their own signature 
a has v' with sender's signature but not one of a (assumption; 1 replicator that does not sign) 
A, b,q2 have 'crashed'
q1 delayed, finally gets v' but not with its own signatures(by assumption the second one)

Sc.3.
A, a, q1,q2 = correct
s, B, b = faulty
s has v signed by itself 
A has v with signature of sender and own signatures 
let a be delayed, a is still waiting for a sender's message (+ the assumption that 1 correct proc that does not sign)
B has 'crashed' 
b has v signed by sender but not by itself
q2 v w sender signature??
Scenario is equivalent to Sc.1, 1 delivers v
B suddenly not crashed anymore, set their value to v' signed by sender and themselves
now let a finally receive a sender's message, v' signed by sender
now let q1 finally receive ?? v' signed
//alternative to this step is b switches to empty (did not sign this round so it's okay)
Any proc must del v

Sc.4.
B, b,q1,q2 = correct
s, A, a = faulty
s has v' signed by itself 
B has v' signed by itself and their signature
let b be delayed, b is still waiting for sender's message (+ aspt 1 corr does not sign)
A - 'crashed'
a has v' signed by sender yet not itself
q1 has v' signed?? or maybe a bit later after delivery
Same as Sc.2; 1 delivers v'
Now A are suddenly not crashed, set to v signed by sender and their own signs
let b finally receive sender's message, v signed by the sender 
let q2 finally receive v signed by sender
//alternative a switches to empty (never appended its own signature this round so fine)
Now same as scenario 3
}



\rmv{


\begin{lemma}
There is no solution to the \rb{} problem on RDMA that tolerates $f < n/2$ failures and in which only the sender signs any messages.
\end{lemma}

\begin{proof}
\Naama{Need to go over this proof. I am not 100\% sure it's correct.}
Assume by contradiction that there exists an algorithm $A$ that solves \neb{} on RDMA in a system with $n = 2f+1$ processes, and does not use any replicator signatures. 
We partition the processes in the system into 4 subsets: $S_1$, $S_2$, $p_1$ and $p_2$, where $\vert S_1 \vert = f$, $\vert S_2 \vert = f-1$, and $p_1$ and $p_2$ contain a single process.
Consider the following scenarios.

\textsc{Scenario 1.} Processes in $S_2$, $p_1$ and $p_2$ are correct, and processes in $S_1$ are faulty, and do not participate. The sender is correct and sends value $v$ to all processes. Then, since the sender is correct and $A$ is a correct algorithm, $p_1$ must eventually deliver $v$. Let $State(p_1)$ be the state of all registers in the set 
$$R_{p_1} = \{r\in R \vert p_1 \text{ was the last process that wrote on } r \text{ before processes in } S_2, p_2 \text{ and } p_1 \text{terminated}\}$$. \Naama{Rephrase to say that these are the registers $p_1$ was the last to write to before some receiver $r$ terminated. (i.e. remove termination from replicators.)}

\textsc{Scenario 2.} Processes in $S_2$, $p_1$ and $p_2$ are correct, and processes in $S_1$ are faulty, and do not participate. The sender is correct and sends value $v'$ to all processes. Then, since the sender is correct and $A$ is a correct algorithm, $p_2$ must eventually deliver $v'$. Let $State(p_2)$ be the state of all registers in the set 
$$R_{p_2} = \{r\in R \vert p_2 \text{ was the last process that wrote on } r \text{ before processes in } S_2, p_1 \text{ and } p_2 \text{terminated}\}$$.

\textsc{Scenario 3.} Processes in $S_2$ and $p_2$ are faulty, the rest are correct. The sender is faulty and sends value $v$ to $p_1$, $v'$ to everyone in $S_1$, and both values to $p_2$ and $S_2$. $S_1$ are delayed, and $S_2$ and $p_2$ act as follows: in all messages sent to $p_1$, and everything written on shared memory, they act identically to their behavior in scenario 1. However, they do not send messages to $S_1$. Note that this scenario is indistinguishable to $p_1$ from scenario 1, so it eventually sends all messages it sent in scenario 1, puts the registers in $R_{p_1}$ in state $State(p_1)$, and delivers $v$. Once $p_1$ delivers, processes in $S_2$ erase all values in all registers not in $R_{p_1}$.  Furthermore, $p_2$ puts all registers in $R_{p_2}$ into state $State(p_2)$, and sends all messages to $S_1$ that it did in scenario 2. At this point in time, processes in $S_1$ start their execution as well. Then, since $p_1$ is correct and delivered $v$, all processes in $S_1$ must eventually deliver $v$ as well.

\textsc{Scenario 4.} Processes in $S_2$ and $p_1$ are faulty, the rest are correct. The sender is faulty and sends value $v'$ to everyone in $S_1$ and $p_2$, and both values to $p_1$ and $S_2$. $S_1$ are delayed, and $S_2$ and $p_1$ act as follows: in all messages sent to $p_2$, and everything written on shared memory, they act identically to their behavior in scenario 2. However, they do not send messages to $S_1$. Note that this scenario is indistinguishable to $p_2$ from scenario 2, so it eventually sends all messages it sent in scenario 2, puts the registers in $R_{p_2}$ in state $State(p_2)$, and delivers $v'$. Once $p_2$ delivers, processes in $S_2$ erase all values in all registers not in $R_{p_2}$.  Furthermore, $p_1$ puts all registers in $R_{p_1}\setminus R_{p_2}$ into state $State(p_1)$, and sends all messages to $S_1$ that it did in scenario 1. At this point in time, processes in $S_1$ start their execution as well.
Note that this scenario is indistinguishable to processes in $S_1$ from scenario 3; the state of the shared memory is the same as it was when they started executing, and they received all the same messages in both scenarios. So, they must deliver $v$. However, this contradicts the agreement property of \rb{}, since $p_2$ was correct and delivered $v'$. 
\end{proof}


\Naama{Stronger lemma we might be able to prove:}

\begin{lemma}
For every replicator $r$ in any solution to the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, there is some execution in which $r$ signs at least one value.
\end{lemma}

\begin{proof}[sketch.]
have an execution in which some correct process $p$ uses $r$ and $f-1$ others in its quorum and terminates.

Another execution in which $q$ does the same but terminates with a different value.

Now we want to claim that if $r$ and the $f-1$ used in $p$'s quorum were Byz, then we can force $p$ into the state it would be upon termination, and then one of the Byz processes (not $r$), would put itself into $q$'s state when it terminated. 

The crux is claiming that any correct process that starts its execution at this point cannot know which of $p$ or $q$ were correct (although it can tell that the processes they used in their quorums were Byz). To make this work, need to think of exactly who needs to be in their quorums (does $q$ have to be in $p$'s quorum to make the numbers work?), and how to convincingly make the states look identical. 

Very similar to the `sender sig is not enough' proof.
\end{proof}

\Naama{Then we should be able to strengthen it to the following lemma:}

\begin{lemma}
In every solution to the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, there is some execution in which a receiver cannot deliver a value $v$ if it sees less than %$2f+1$ unsigned values and 
$f+1$ signed values.
\end{lemma}

\begin{proof}
Assume by contradiction there is some algorithm $A$ that solves the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, in which there is no execution such that a receiver $r$ delivers a value $v$ after it saw at least $f+1$ signatures from different replicators.

Let $S$ be the set of $f$ replicators that produced signatures that $r$ saw, let $p$ be the replicator that did not communicate with $r$ at all, and let $S'$ be the set of $f$ replicators that communicated with $r$ but did not produce any signatures. Let $r'$ be another receiver.

\textsc{Scenario 1.} 

\textsc{Scenario 2.} Everyone in $S'$ is Byzantine. After $r$ terminates they erase their state and put themselves into the state they should be in if they received $v'$ from the sender, signed the values, and $S$ never wrote anything. \Naama{For this to work, I think we also need to get the correct replicator $p$ to have $v'$.}
\end{proof}

\Naama{This lemma should imply the following:}

\begin{lemma}
For every solution to the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, there is some execution in which all replicators sign at least once.
\end{lemma}

\begin{proof}[sketch.]
\Naama{This proof assumes that the correct behavior for some processes is not to sign in this execution. We need to show that if not everyone signs, then this behavior is correct under the execution we are showing.}

Assume by contradiction there is some algorithm $A$ that solves the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, such that there is no execution of $A$ in which all replicators sign.

Consider partitioning the processes into 5 sets, $C$, $c$, $B$, $b$, and $p$ where $|C| = |B| = f-1$, and $|c|=|b|=|p| = 1$.
Consider the following scenarios.

\textsc{Scenario 1.} $C$, $c$, and $b$ are correct, and the rest are faulty. The sender is correct and sends value $v$ to all. The faulty processes don't participate.
Note that in this scenario, there must be at least one correct process that does not sign, since this is indistinguishable to the correct processes from an execution in which all the faulty processes append their signatures after the correct ones sign. Let the correct process that doesn't sign be $b$. Then by the termination property of reliable broadcast, a receiver must be able to deliver $v$ in this execution.

\textsc{Scenario 2.} $B$, $b$, and $c$ are correct, and the rest are faulty. The sender is correct and sends $v'$ to all. The faulty processes don't participate. Similarly to the previous scenario, there must be some correct process that doesn't sign. Let that correct process be $c$. Then by the termination property of reliable broadcast, a receiver must be able to deliver $v'$ in this execution.

\textsc{Scenario 3.} $C$, $c$, and $p$ are correct, the rest are faulty. Furthermore, the sender is faulty, and sends $v$ to the correct processes, and both values ($v$ and $v'$) to the faulty processes. Processes in $B$ and $p$ are silent at first, and $b$ pretends to be correct and to have received only $v$, and participates in the protocol until $C$ and $c$, reach the same state of Scenario 1 at the point in time a receiver could terminate. At this point, this Scenario is indistinguishable to the receiver from Scenario 1, so it delivers $v$.

Now, $b$ erases its value, and all faulty processes (in $B$ and $b$) put themselves into the same state of Scenario 2, pretending to have seen values supporting $v'$, but with no signatures, from process $c$. At this point $p$ may wake up and do whatever the protocol dictates for it. 
In this scenario, any receiver that observes the state at this point must deliver $v$, since a receiver before it delivered $v$.

\textsc{Scenario 4.} This scenario is analogous to Scenario 3. This time, $B$, $b$, and $p$ are correct, and the rest are faulty. The sender sends $v'$ to processes in $B$ and $b$, $v$ to $p$, and both values to the faulty ones. $p$ and $C$ are silent at first, $c$ pretends to be correct and have received value $v'$, until $B$ and $b$ reach the state of Scenario 2. At this point, this is indistinguishable to a receiver from Scenario 2, so it delivers $v'$.

Now, $c$ erases its value, and all faulty processes (in $C$ and $c$) put themselves into the same state of Scenario 1, pretending to have seen values supporting $v$, but with no signatures, from process $b$. At this point $p$ may wake up and do whatever the protocol dictates for it. Note that the state of all processes when $p$ wakes up in this Scenario is indistinguishable from the state $p$ observed in Scenario 3, so $p$ must do the same thing it did in Scenario 3.
In this scenario, any receiver that observes the state at this point must deliver $v'$, since a receiver before it delivered $v'$. However, this scenario is indistinguishable from Scenario 3, leading to a contradiction in agreement if they deliver, or a contradiction in termination if they don't.
\end{proof}


Attempt 2, assuming that the following lemma is also true:


\begin{lemma}
In every execution in which only $f+1$ replicators participate and the sender is correct, at least one replicator must sign.
\end{lemma}

\begin{proof}
Assume by contradiction that this claim does not hold. Then, there exists an execution $E$ in some algorithm $A$ that solves reliable broadcast on RDMA and tolerates $f \leq n/2$ failures, such that only $f+1$ replicators participate in $E$, the sender is correct, and no replicator signs. Without loss of generality, assume the value that the sender sends in $E$ is $v$.

Let the set of replicators that participate in $E$ be $C$. Consider the following execution, $E'$ of $A$. In $E'$, $C \setminus \{c\}$ are Byzantine, and the rest of the replicators are correct. Furthermore, the sender is faulty, and sends the value $v$ to $c$, $v'$ to all other correct replicators, and both values to $C\setminus \{c\}$. The processes in $C$ behave correctly and pretend to have received value $v$ from the sender, until a time where a receiver delivers $v$. Such a time must exists since the prefix of $E'$ is indistinguishable from $E$, and $A$ tolerates  $f \leq n/2$ replicator failures and the sender is correct in $E$.

At this point, $C \setminus \{c\}$ erase their values, and $c' \in C \setminus \{c\}$ pretends to wake up now and have value $v'$ from the sender. Furthermore, all correct replicators other than $c$ wake up and start their execution as well.
\Naama{This proof should actually be identical to the proof that it's not enough for the sender to sign.}
\end{proof}

\begin{lemma}
Let $A$ be an algorithm solving reliable broadcast on RDMA tolerating $f \leq n/2$ failures, such that no execution of $A$ has all $n$ processes signing.
Then in every execution of $A$, there exist two disjoint sets $S_1$ and $S_2$ and two elements $s_1 \in S_1$ and $s_2 \in S_2$ such that $|S_1| = |S_2| = f$, and 
(1) in an execution in which only $S_1$ and $s_2$ participate and receive input $v$, $s_2$ doesn't have to sign, and 
(2) in an execution in which only $S_2$ and $s_1$ participate and receive input $v'$, $s_1$ doesn't have to sign.
\Naama{Proving this boils down to a combinatorial problem. If we can prove this lemma, then we've proven our lower bound.}
\end{lemma}

\begin{lemma}
For every solution to the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, there is some execution in which all replicators sign at least once.
\end{lemma}

\Naama{We're gonna try to make $b$ and $c$ always be part of the set that we know doesn't have to sign for that particular execution. Need to see if it always works out. Might need to use $p$ in some places.}
\begin{proof}
Assume by contradiction there is some algorithm $A$ that solves the \rb{} problem on RDMA tolerating $f\leq n/2$ failures, such that there is no execution of $A$ in which all replicators sign.

Consider partitioning the processes into 5 sets, $C$, $c$, $B$, $b$, and $p$ where $|C| = |B| = f-1$, and $|c|=|b|=|p| = 1$.
Consider the following scenarios.

\textsc{Scenario 1.} The set $C$, where $|C| = f$ is correct. Additionally, one more process, $p$ is correct. The rest of the replicators are faulty and don't participate. The sender is correct and sends $v$ to all processes. By Lemma~\ref{lem:manydontsign}, at least one correct process does not sign during this execution. Without loss of generality, let $p$ be a process that doesn't sign.
Then, by the termination property of \rb{}, some receiver eventually delivers $v$.

\textsc{Scenario 2.} A different set of processes, $C'$, where $|C'| = f$ is correct, where the intersection between $C$ and $C'$ is empty, but $C'$ contains $p$. There is one more correct process, $q$. The sender is correct and sends $v'$ to all. The rest of the processes are faulty and don't participate. 

We pick $q$ such that in this execution, $q$'s correct behavior is not to sign. We know that $q$ exists by Lemma~\ref{lem:manydontsign}; in every execution, there are at least $f+1$ processes whose correct behavior is not to sign, so there is some process $q$, $q\not\in C'$, such that $q$ does not sign during this execution. Furthermore, by Lemma~\ref{lem:onesig}, at least one process 

So, by the termination property of \rb{}, some receiver eventually delivers $v'$.

\textsc{Scenario 3.} $C$ and another process $s\not \in C'$ are correct, the rest are faulty. Furthermore, the sender is faulty, and sends $v$ to the correct processes, and both values ($v$ and $v'$) to the faulty processes. Processes in $C'\setminus \{p\}$ and $s$ are silent at first, and $p$ pretends to be correct and have received $v$ and participates in the execution. Then, eventually, we reach a state indistinguishable from Scenario 1.  So, a receiver may deliver $v$ at this point.

After this happens, processes in $C'$, including $p$, put themselves in the same state they got to in Scenario 2. At this point, $s$ wakes up and does whatever the protocol dictates.
Any receivers observing this state must deliver $v$, to satisfy agreement.

\Naama{Can we make $q$ be a part of set $C$? If so, this proof should be identical to the previous proof.}

\textsc{Scenario 4.} This scenario is analogous to Scenario 3. This time, $C'$ and $s$ are correct, and the rest are faulty. The sender sends $v'$ to correct processes, and both values to all others. $q$ participates and pretends to be correct and have received value $v'$. Then eventually we get to the same state as Scenario 2, and some receiver delivers $v'$.

We now consider two cases.
Case 1: $q \neq s$. Then, since $|C| = |C'| = f$, $q\not\in C'$, and $s \not \in C$ and $s\not \in C'$, $q$ must be in $C$, and $q$ is faulty. In this case, all processes in $C$ now put themselves in the state they were in in Scenario 1.

At this point, $s$ wakes up and does whatever the protocol dictates.
This scenario is indistinguishable from Scenario 3, meaning that receivers at this point must deliver $v$. However, this breaks agreement.

Case 2: $q = s$. Then $q$ is correct. This leads to a problem, since even if $C$ put themselves in the state of Scenario 1, this is not indistinguishable from Scenario 3.
\end{proof}
}

\rmv{
\Naama{Other things we'd like to prove:
\begin{enumerate}
    \item for \rb{}, there is some execution in which each replicator needs to create at least two signatures
    \item Any solution to \rb{} has some execution with at least 4 message dependencies 
    \item In any solution to \rb{} that has some execution with 2 message dependencies, some execution must have at least 5 message dependencies
    \item For the consensus story: show that under conditions that trigger the slow path for \rb{}, but do not trigger a view change, we can't make a `middle path' for \rb{} that's as fast as \neb's slow path.
\end{enumerate}
}

\Naama{Questions/notes/ideas for story:
\begin{itemize}
    \item how many signatures are introduced in the pbft implementation that uses \neb{}, outside of \neb{} itself?
    \item if the answer to the above is good (i.e. not many), we could potentially make the `broadcast for consensus' story without any of the message dependency results (saves us having to prove points 2-4 above), and instead focus on the advantage of using a weaker abstraction like \neb{} instead of a stronger one like \rb{} in terms of just the number of wasted signatures.
    \item for this signature-based story, need to make a strong case for why signatures are expensive. Not only plots produced on current machines, but also addressing the claims that soon there will be a way to produce and verify signatures at line rate.
\end{itemize}}
}


